Feature selection in high-dimensional dataset using MapReduce

This paper describes a distributed MapReduce implementation of the minimum Redundancy Maximum Relevance algorithm, a popular feature selection method in bioinformatics and network inference problems. The proposed approach handles both tall/narrow and wide/short datasets. We further provide an open source implementation based on Hadoop/Spark, and illustrate its scalability on datasets involving millions of observations or features.

==> associative <==
M: a  +  b  +  c  +  d
     \   /      \   /
C:  (a+b)=S1   (c+d)=S2
             \         /
R:         ( S1 + S2 )


==> associative2 <==
M:   a  +  b  +  c  +  d
      \   /       \   /
R:  ((a+b)   +   (c+d))


==> map <==
// The mapper input is $\left(\bar{x}_{i_{c}}, \bar{x}_{i_{s}}, c_i\right)$
for each $x_k \in \bar{x}_{i_{c}}$:
  output($k$, ($x_k$, $c_i$, $id$))
  for each $x_j \in \bar{x}_{i_{s}}$:
    output($k$, ($x_k$, $x_j$, $id$))


==> random <==
getResult($\cdot$)
  return random_scalar_value()


==> reduce <==
// The reducer input is ($k$, list(($x_k$, $v$, $id$)))
if is_target_feature($v$, $id$):
  compute $I_{x_{k}, c} \leftarrow I\left(x_{k}, v\right)$
else
  compute $I_{x_{k}, x_{id}} \leftarrow I\left(x_{k}, v\right)$
mRMR Score($x_{k}$) $\leftarrow$ $\begin{cases}
I_{x_{k}, c} - \sum_{x_{id}} I_{x_{k}, x_{id}} & \left|I_{x_{k}, x_{id}}\right| \leqslant 1 \\
I_{x_{k}, c} - \frac{1}{\left|\bar{x}_{s}^{l}\right|-1} \sum_{x_{id} \in \bar{x}_{s}^{l}} I_{x_{k}, x_{id}} & \left|I_{x_{k}, x_{id}}\right| > 1
\end{cases}$
output($k$, mRMR Score($x_{k}$))

